Bounded-Memory Strategies in Partial-Information Games

We study the computational complexity of solving stochastic games with mean-payoff objectives. Instead of identifying special classes in which simple strategies are sufficient to play $\epsilon$-optimally, or form $\epsilon$-Nash equilibria, we consider general partial-information multiplayer games and ask what can be achieved with (and against) finite-memory strategies up to a {given} bound on the memory. We show $NP$-hardness for approximating zero-sum values, already with respect to memoryless strategies and for 1-player reachability games. On the other hand, we provide upper bounds for solving games of any fixed number of players $k$. We show that one can decide in polynomial space if, for a given $k$-player game, $\epsilon\ge 0$ and bound $b$, there exists an $\epsilon$-Nash equilibrium in which all strategies use at most $b$ memory modes. For given $\epsilon>0$, finding an $\epsilon$-Nash equilibrium with respect to $b$-bounded strategies can be done in $FN[NP]$. Similarly for 2-player zero-sum games, finding a $b$-bounded strategy that, against all $b$-bounded opponent strategies, guarantees an outcome within $\epsilon$ of a given value, can be done in $FNP[NP]$. Our constructions apply to parity objectives with minimal simplifications. Our results improve the status quo in several well-known special cases of games. In particular, for $2$-player zero-sum concurrent mean-payoff games, one can approximate ordinary zero-sum values (without restricting admissible strategies) in $FNP[NP]$.

==> NPhardness.tex <==
We will in this section show that approximating the value of an imperfect-information 1-player reachability game is NP-hard and coNP-hard, even when the player is restricted to using memory-less strategies. Indeed, we show that an  optimal strategy exists and is memory-less and does not use randomization. 
\newcommand{\INIT}{\mathop{INIT}}
\newcommand{\WIN}{\mathop{WIN}}
\newcommand{\LOSE}{\mathop{LOSE}}
\newcommand{\TRUE}{\mathop{true}}
\newcommand{\FALSE}{\mathop{false}}
\begin{theorem}
Approximating the value of an imperfect-information 1-player reachability game is NP-hard and coNP-hard, even when the player has an optimal memory-less, deterministic strategy in that game. 
\end{theorem}

\begin{proof}
We will first show that it is NP-hard to decide if the value of a game is high enough.

The reduction will be from 3SAT: You are given a boolean CNF formula with 3 literals per clause, i.e. \[
\bigwedge_{j=1}^m \bigvee_{k=1}^3 v_{k,j}
\]
where $v_{k,j}$ is a variable in $\{v_i,\neg v_i\mid i\in {1,...,n}\}$. 
A truth assignment is an assignment to each variable $v_i$ for $i=1$ to $n$ of either true or false. Assigning true to $v_i$ makes $\neq v_i$ false. 
A clause $j$ is satisfied by a truth assignment if one of $\{v_{1,j},v_{2,j},v_{3,j}\}$ is assigned true by the assignment.
A CNF formula is true if there is an assignment such that each clause $j$ is assigned true by it. 3SAT is the question of whether, given a CNF formula, is it true? 3SAT is one of the most well-known NP-complete problems and is in particular NP-hard. 

We now describe the corresponding game.
The game consists of states \[
\{\INIT\}\cup\{(i,j)\mid i\in \{1,...,n\},j\in \{1,...,m\}\}\cup\{\WIN_2,...,\WIN_{n+1}\}\cup\{\LOSE\}
\]
$\INIT$ is the initial state. 

There is a single action from $\INIT$ that goes to each of $\{(1,j)\mid j\in \{1,...,m\}\}$, and assigns uniform probability to each successor state.
From $(i,j)$ there are two actions, $\TRUE$ and $\FALSE$, each deterministic. $\TRUE$ goes to $\WIN_{i+1}$ if $v_i$ is in $\{v_{1,j},v_{2,j},v_{3,j}\}$ and otherwise to $(i+1,j)$ if $i<n$ and otherwise, if $i=n$ and $v_i$ is not in $\{v_{1,j},v_{2,j},v_{3,j}\}$, it goes to $\LOSE$. Similarly, $\FALSE$ goes to $\WIN_{i+1}$ if $\neg v_i$ is in $\{v_{1,j},v_{2,j},v_{3,j}\}$ and otherwise to $(i+1,j)$ if $i<n$ and otherwise, if $i=n$ and $\neg v_i$ is not in $\{v_{1,j},v_{2,j},v_{3,j}\}$, it goes to $\LOSE$.
From $\WIN_{i}$ for $i<n+1$, there are similarly two actions, $\TRUE$ and $\FALSE$, both going to $\WIN_{i+1}$. 
From $\WIN_{n+1}$ and $\LOSE$ respectively there is a single action going to themselves. 
 
The player's single in $\INIT$ is $0$, and in $(i,j)$ and $\WIN_i$ it is $i$ and in $\LOSE$ it is $n+1$.
In particular, in round $i$, the signal is $\min(i,n+1)$ (counting from 0). 

The reward in the action in $\WIN_{n+1}$ is 1 and all other rewards are 0. In particular, the game is a reachability game, because the only way to get a non-0 reward is to get to $\WIN_{n+1}$ and if you do reach $\WIN_{n+1}$ the rest of the rewards will be 1.

Consider the truth assignment that maximizes the number of clauses it satisfies and let that number be $b$. 
We will argue that the value of the game is $b/m$ and that there is a memory-less deterministic strategy ensuring so. In particular, the value is 1 if the CNF formula is true and otherwise, it is at most $1-1/m$. 

Observe that we can for each play of length $n+1$ identify a truth assignment, i.e. the one that assigns $v_i$ to true if and only if the action in round $i$ was $\TRUE$. We can see that a play reaches $\WIN_{n+1}$ if and only if it went into a state $(1,j)$, for some $j$ in round 1 and clause $j$ is satisfied by the truth assignment identified by the play. 

Consider some assignment that satisfies $x$ clauses for any $x$. We can then translate it into a memory-less deterministic strategy for the player that plays $\TRUE$ on signal $i$ if $v_i$ is true in the assignment and $\FALSE$ otherwise. This strategy wins the game with probability $x/m$, because in round $0$, nature picks uniformly at random a state $(1,j)$. In $x$ cases (the ones where $j$ is some clause satisfied by the assignment), the resulting play leads to $\WIN_{n+1}$ and in the remaining cases to $\LOSE$. Thus, the probability to win is $x/m$. In particular, the memory-less deterministic strategy that corresponds to a truth assignment satisfying $b$ clauses has a probability of $b/m$ of winning.

Consider any strategy for the player (using an arbitrary amount of memory).  Since the history of signals in a play is always $0,1,2,...,i$ in round $i$ for $i\leq n+1$ (looping with $n+1$ for bigger $i$'s) we can view this strategy as a probability distribution over truth assignments (the ones identified by the resulting plays). Any individual truth assignment can win with probability at most $b/m$, by definition of $b$. Therefore, any distribution over truth assignments can win with probability at most $b/m$. 

Hence, it is NP-hard to decide if the value of such a game is $1$ and coNP-hard to decide if the value of the game is at most $1-1/m$, even though the value is either $1$ or $1-1/m$ or below. Therefore, it is NP-hard and coNP-hard to approximate the value within $\pm x$, for $x<1/(2m)$.
\end{proof}




==> app.FOR.tex <==
We assume familiarity with \FOR, the first order theory of the reals \cite{BPR2006},
and will make repeated use of the fact that one can bound satisfying evaluations, if they exists.
The following states this formally. %

\thmFORbounds*
\input{thm.big-number-solutions}



==> app.move-me.tex <==
\subsection{move me} 
\begin{remark}\emph{Is this trivial for computational complexity?}
If one ignores how small the probabilities involved might be, the complexity classes for the approximation results seem natural or perhaps even a bit high: E.g. for $\epsilon$-Nash equilibria, we guess an $\epsilon$-Nash equilibria and then check if any possible strategy we could replace with would be an improvement. This is actually what we end up doing, but we cannot ignore how small the probabilities might be. Indeed, already for the 2-player, zero-sum, concurrent reachability special case, there are $\epsilon$-optimal stationary strategies\cite{} or equally stationary $\epsilon$-Nash equilibria (i.e. the bound on the memories are 1), but in some games, each such strategy uses at least double exponentially small positive numbers\cite{}! We do show that double exponentially small do suffice even in general, see \ref{}, but it does mean that we can not write the strategies with probabilities in binary, so instead we write them using floating point numbers, which we can then insert into our game and get a Markov chain. Since the numbers are written as floating point numbers we then proceed to give an algorithm for finding the outcome of Markov chains with such. Because of the floating point numbers, we only give an approximation algorithm, however. 

One might think that (at least in special cases) we should be able to use that best responses ``should be'', intuitively speaking, memoryless, deterministic or in particular locally optimal (defined using e.g. potentials like those used by the strategy iteration framework for e.g. turn-based or concurrent games). However, because we can only approximate the outcome due to the floating point numbers, this intuition breaks down in regards to the local optimality: Indeed something close to locally optimal might be very far from globally optimal (e.g. you have a long list of repeated local changes before you get to the global optimal and while perhaps each might be small, the total change might still be big). In some special cases, we can as such use the memoryless-ness or that they should be deterministic, but we would need to search through all the exponentially many such strategies anyway so it would not lead to a better computational complexity class.
\end{remark}



\paragraph{Arena}
The arena consists of a graph, where each state belongs to some player. Plays of such an arena then start with a pebble on some state, which is then in each round moved to a successor state by the owner of the state the pebble is on currently. A finite-memory strategy then means that there is a finite set of memory states, and is followed if the player always moves the pebble according to a distribution depending on the current memory together with their observation of the current state, after which each player updates their memory according to a distribution based on their current memory and their observation of the move. A strategy is public if each player can observe the current memory of the strategy (i.e. when picking a move/updating their memory). Partial observation is then that some states and/or moves might look the same - exactly what looks the same for each player is specified as part of the game. 


\paragraph{Objectives}
Given a play in such an arena, the objectives define the expected outcome for each player. There are several standard objectives often considered, including mean-payoff, parity, reachability and discounted objectives, see the preliminaries for definitions.


\paragraph{Equilibria and optimality and restricted notions of such}
For any $\epsilon\geq 0$, a $\epsilon$-Nash equilibria of a game is strategy profile (=a set of strategies, one for each player), so that each player can at most improve their expected outcome by $\epsilon$ by replacing their strategy with another strategy (resp. with another strategy in $S$). A strategy is $\epsilon$-optimal if there is a $v$ so that for all strategy profiles containing it, the player's expected outcome is at least $v$ while replacing the strategy with another strategy and for all strategy profiles containing that strategy, the outcome is at most $v+\epsilon$. 

We are interested in restricted notions of $\epsilon$-Nash equilibria and $\epsilon$-optimal strategies. In the restricted notions, we have a set of strategy profiles and the players can only replace their strategy with other strategies from that set.



==> imp-pomdps.tex <==
For partial information one-player games, aka partially observable Markov decision processes (POMDPs), \citeauthor{MHC1999} \cite{MHC1999}
showed that it is undecidable to check if the game value exceeds a given threshold.
This is true even for the special case of reachability objectives and 
when the player is ``blind'' (there is only one possible signal).
On the other hand, for POMDPs with mean-payoff objectives, there always exist finite-memory strategies that are $\eps$-optimal \cite{CSZ2022}.
Together with \cref{thm:main-1}, this means there cannot be a computable bound on the memory of $\eps$-optimal strategies for a given $\eps$ and POMDP $G$.
This result is already implied by \citeauthor{CSZ2022}\cite[Remark 3.3]{CSZ2022} for pure strategies.
\sbnote{Please check this and confirm}


==> imp-pozs.tex <==
These games are not guaranteed to be determined and previous work has focused on finding special cases where this issue can be avoided.
In particular, \citeauthor{HPPR2018} \cite{HPPR2018} identify subclasses where the value can be witnessed
by ``cycle-forming'' strategies, which use at most $2^{\card{\states}}$ memory modes,
or memoryless strategies.
They show that determining if the value of a \emph{forcibly first abstract cycle games} exceeds a given threshold is in \PSPACE. The fact that these games admit 


In the former case, our results do improve state of the art for some such results, such as~\cite{HPPR2018}, but they, like in some other cases, further ensure that positional strategies suffice, which makes \NP$\cap$\coNP\ trivial.



==> sec.alg-mc.tex <==
A Markov chain with mean-payoff objective is a $0$-player game given by a set of states $\states=\{1,\dots,n\}$ with a unique action $a\in \actions$. Due to the uniqueness of action, we write $\probm(i,a)(j)$ as $\probm(i,j)$ as the probability of the edge from $i$ to $j$.
Each edge also has a reward and duration denoted by $\rew(i,j)$ and $\dur(i,j)$ respectively. %
A state $i\in \states$ is called an \emph{absorbing} state if $\probm(i,i)=1$, otherwise it is \emph{transient}. 
\ptnote{ordinarily, transient is "not recurrent", meaning that the chance of revisiting it \emph{eventually} is not 1}

We are interested in computing the expected \emph{mean-payoff ratio} of a given initial state in a Markov chain. Recall that the {\mpr} of an infinite play $\play=s_0s_1\ldots$ is
\[
    \avgrew(\rho) = \liminf_{N\to\infty} \frac{\sum_{i=0}^N \rew(i,i+1)}{\sum_{i=0}^N\dur(i,i+1)}
\]
Clearly, this corresponds to the usual \mpo\ if all edges have duration one.

A \emph{bottom strongly connected component (BSCC)} of a Markov chain is a subset of vertices $S\subset \states$ such that for every $i,j\in S$, a play starting from $i$ reaches $j$ with probability $1$.
This gives for every pair $i,j\in S$, a expected duration and expected reward of going from $i$ to $j$.
\ptnote{move def of BCC into main text (is used)}
\ptnote{below could be shortened by sing some references in proofs?}
Assuming that all states are reachable from the initial state with positive probability, it is easy to see that a play starting from any state of a Markov chain will reach an BSCC with probability $1$. This is because the probability of a state repeating $k$ times decreases as $k$ increases unless the state is part of an BSCC. Therefore, the likelihood of plays which only visit states not in any BSCC is $0$. This means that the play eventually reaches an BSCC and therefore the mean-payoff value can be expressed as the sum of mean-payoff value of all BSCCs weighted by the probability of reaching the BSCC from the initial state.

\paragraph{Cycle Mean-payoff value}
 For a run $s_1,s_2,\dots $ 
 \ptnote{runs or plays? sequences of edges?}
 starting in an BSCC $S$, and a marked state $s\in S$, we define the $s$-cycle mean-payoff reward of the run as $\frac{\sum_{i=\ell}^{k}\rew(s_i,s_{i+1})}{\sum_{i=\ell}^{k}\dur(s_{i},s_{i+1})}$, where $s_\ell=s_{k+1}=s$ and $s_i\neq s$ for all $\ell< i <k+1$. In other words, the run is cut off once a cycle is reached on state $s$ and the average mean payoff ratio from the edges in the cycle are counted.
The $s$-cycle mean-payoff value is defined as the limit of the expected $s$-cycle mean-payoff ratio value of runs of increasing lengths. It is easy to see that as the length increases, the probability of not visiting a $s$-cycle decreases and in the limit, converges to $0$. The following lemma proves that for a BSCC Markov chain, i.e, all states are part of a single BSCC, the mean-payoff value is equal to the $s$-cycle mean-payoff value, for any state $s\in S$.

\begin{lemma}
	\label{lem:cycle-mean-payoff}
	The mean-payoff value of a BSCC Markov chain is equal to the $s$-cycle mean-payoff value, for any state $s\in S$, for any choice of initial state.
        \ptnote{can we avoid ``BCC MC'' and spell this requirement out?
        And also add in the other assumptions on the MC? (bounded rew/step)}

\end{lemma} 

\begin{proof}
	Fix a state $s\in S$ and a initial state $s_0\in S$. Let $d_0$ be the expected duration of going from $s_0$ to $s$, and $d_s$ be the expected duration of completing a cycle from $s$ to $s$. By the Markov inequality, the probability of a run from $s_0$ to $s$ of duration $\geq \frac{d_0}{\eps/4}$ is $\leq \eps/4$. 
        \ptnote{any reason why we don't write $4d_0/\eps$ and similarly later?}
	Similarly, the probability that a run starting from $s$ does not reach $s$ in duration $\frac{d_s}{\eps/4}$ is $\leq \eps/4$. 
	Therefore, we can consider runs of a fixed duration $d_X>\frac{d_0}{\eps/2}+X\frac{d_s}{\delta}+ \frac{d_s}{\eps/2}$, where $\delta=\eps/X$, which consists of three parts as follows:
	\begin{itemize}
		\item a prefix from $s_0$ to $s$ in duration at most $\frac{d_0}{\eps/2}$, 
		\item have at least $X$ number of $s$-cycles each of which has duration at most and $\frac{d_s}{\delta}$, where $\delta=\eps/X$,  and
		\item a $s$-cycle free suffix from last occurrence of $s$ of duration $\leq \frac{d_s}{\eps/2}$.
	\end{itemize}
	All other runs which do not satisfy the conditions for prefix and suffix have probability $\leq \eps$ by the union bound. A similar argument bounds the probability of the run satisfying all of the above conditions by $\eps+\delta$. 
        \ptnote{you mean $1-\eps-\delta$? (We need the complement of the above?)}
        Therefore, we now focus on runs in which, prefix, cycles and suffix are all of bounded lengths.
	
	The total reward of such runs is the sum of the reward in the prefix, suffix and the $s$-cycles. Since the prefix and suffix are of length at most $\frac{d_0}{\eps/2}+\frac{d_s}{\eps/2}$, the reward obtained in the prefix and suffix can be upper bounded by $B(\frac{d_0}{\eps/2}+\frac{d_s}{\eps/2})$, where $B$ is the bound on reward per unit time. Note that this is constant as $d_X$ tends to $\infty$. Therefore, we can consider only the reward accumulated in the $s$-cycles in the mean-payoff value. 
	The duration of a play completing at least $X$ cycles of duration $d_X$ is at most $\frac{d_0}{\eps/2} + (X)\frac{d_s}{\delta} + \frac{d_s}{\eps/2}$. 
	
	At most $\frac{d_0}{\eps/2}+\frac{d_s}{\eps/2}$ part of the duration is spent in the prefix from $s_0$ to $s$ and a $s$-cycle-free path starting from $s$ which can be bounded by a constant $C$. 
	The mean-payoff value of such a play of duration $d_X$ is
	$\frac{1}{d_X} (\rew_{\text{prefix}} + \rew_{\text{loop}}  + \rew_{\text{suffix}})$. 
        Note that the loop part of runs have at least $X$ occurrences of the loops. Therefore, $\rew_{\text{loop}}$ can be written as sum of each \emph{simple} cycle, of which there are at least $X$ of them. The duration $d_X$ can be written as the durations of the simple cycles plus at most $C$ for the duration of the prefix and suffix. The mean-payoff value can therefore be expressed as the limit of the expected reward divided by expected duration of simple cycles and prefix and suffix as $X$ increases. As $X$ increases the expected duration of the prefix and suffix remains bounded. By law of large numbers, as $X$ tends to $\infty$,  the mean payoff value tends to  $\frac{X\expectation(\rew(\text{loop}))}{C+ X\expectation(\dur(\text{loop}))}$. In the limit, this is the same as $\frac{X\expectation(\rew(\text{loop}))}{X\expectation(\dur(\text{loop}))}$ which is the expected cycle mean-payoff reward. This completes the proof.
        \ptnote{spell this equality out in a math env}

\end{proof}





 As a corollary, we also obtain that the mean-payoff value is the same in all states of the BSCC.
This proves that the mean-payoff value in a BSCC can be replaced by the $s$-cycle mean-payoff value, for any state $s$ of the BSCC. 
  

\paragraph{Allowing multiple edges}
As an intermediate model we allow multiple (possibly countably infinitely many) edges $e_1,e_2,\dots$ between a pair of states $i,j$ and write $\probm(e)$, $\rew(e)$ and $\dur(e)$ to denote the associated probability, reward and duration for edge $e$.
We have the additional assumption that reward per unit duration is upper bounded. Also, since there are countably many edges, the durations and rewards of an edge can no longer be bounded by the maximum of them. We instead assume that the expected reward and duration to go from $i$ to $j$ is finite for any pair $i,j$ is bounded. This gives a upper bound on the expected duration between any pair of state.

Note that Lemma \ref{lem:cycle-mean-payoff} works even with the multiple edge definition of 
\ptnote{can we make this explicit in the statement of the lemma?}
Markov chains with the above assumptions. The last assumption is used to say that for a $k$-step run, the probability that the duration of this run being $>2D$ is small, where $D$ is an upper bound on the expected duration to go from $i$ to $j$. The first assumption is used to bound the loss in reward going from the reward in the run to the reward in the loop part of the run. Therefore, we can work with the cycle mean-payoff value even in the case where there are countably many edges between a pair of states under the above assumptions. The following lemma states that multiple edges between a pair of states $i,j$ can be combined into one edge without changing the mean-payoff value.



\begin{lemma}[Edge Collapse]
	\label{lem:edge-collapse}
	Let $M$ be a Markov chain with edges $e_1,e_2,\dots $ from state $i$ to $j$. Let $M_c$ be the Markov chain obtained by replacing $e_1,e_2,\dots$ by an edge $e$ with
        \ptnote{the $c$ in $M_c$ is not a number; let's use $M'$ as in other places?}
	\begin{itemize}
		\item $\probm(e)= \sum_i \probm(e_i)$
		\item $\rew(e)= \sum_i (\probm(e_i)\rew(e_i))$
		\item $\dur(e) = \sum_i (\probm(e_i)\dur(e_i))$
	\end{itemize}
Then $M$ and $M_c$ have the same cycle mean-payoff value from the initial state.
\end{lemma}
\begin{proof}
If $i$ is not in a BSCC, then the probability of reaching a BSCC is preserved by collapsing the edges.  If $i$ is in a BSCC, we prove that the $i$-cycle mean payoff value is $M$ and $M_c$ is the same. 
\ptnote{a figure to illustrate the countably inf edges?}

Consider a cycle starting from $i$ in $M_c$. If the outgoing edge from $i$ is not the collapsed edge $e$, then the same cycle exists in both $M$ and $M_c$ and have the same rewards, duration and probability.
Now, consider a cycle $c = e \play$, such that $\play$ is a path from $j$ to $i$. Define $c_i = e_i\play$. By definition, the expected reward (or duration) from the play $c$ in $M_c$ is the sum of expected reward (respectively duration) from $e$ and the expected reward (respectively duration) from plays that are simple paths  from $j$ to $i$.
The expected reward (respectively duration) from cycles $c_i$ in $M$ will be the expected reward (respectively duration) in the first edge and from the rest of the play. The second part is the same in both $M$ and $M_c$ and by construction, the reward (respectively duration) from $e$ is the expected reward (respectively duration) from the edges $e_i$, for all $i$. Therefore, the BSCC containing $i$ has the same mean-payoff value in $M$ and $M_c$.	
\end{proof}

We now give an algorithm to compute the mean-payoff value in Markov chains by iteratively reducing the state-space. This is done by alternating two operations, state and loop elimination, described in the next subsections.  

\subsection{State Elimination}
\begin{figure*}[t]
  \centering
  \input{fig/se-full.tikz}
  \caption{State elimination:
  On the left is (part of a) Markov chain $M$ before removing state $n$ and on the right is the corresponding part of Markov chain $M'$. In the middle is the intermediate step $M''$ as constructed in the proof of \cref{lem:state-elim}. The probability, and expected duration and reward, of moving from state $i$ to $j$ remains untouched.}
  \label{fig:state_elim_full}
\end{figure*}
	
The state-elimination step takes as input a Markov chain with states $\{1,\dots,n\}$, where $\probm(n,n)=0$ and produces a Markov chain $M'$ with states $\states'=\states \setminus \{n\}$. %
where, for every pair of state $i,j\neq n$, the values of probabilities, rewards, and durations are updated as follows:
\begin{align*}
    \probm'(i,j) &\qquad\eqdef\qquad \probm(i,j) + \probm(i,n)\cdot \probm(n,j)\\
    \rew'(i,j)   &\qquad\eqdef\qquad \probm(i,j)\rew(i,j) + \probm(i,n)\cdot \probm(n,j)(\rew(i,n)+\rew(n,j))\\
    \dur'(i,j)   &\qquad\eqdef\qquad \probm(i,j)\dur(i,j) + \probm(i,n)\cdot \probm(n,j)(\dur(i,n)+\dur(n,j))		
\end{align*}

\stateelim*

\newcommand{\auxM}{M''}
\begin{proof}
	We prove this in two steps. First we construct an intermediate Markov chain $\auxM$, 
        which contains a new edge for any length-$2$ path via the state $n$ that will be eliminated. That is, 
        for every pair of states $i,j\neq n$, two edges $e_{ij}$ and $e'_{ij}$. The probability, reward and duration of edge $e_{ij}$ are equal to $\probm(i,j)$, $\rew(i,j)$ and $\dur(i,j)$ respectively. 
	The probabilities, rewards and durations of edges $e'_{ij}$ are obtained as follows
        (see also \cref{fig:state_elim_full} in the middle).
        \begin{align*}
	    \probm(e'_{ij}) &\qquad\eqdef\qquad  \probm(i,n)\probm(n,j)\\
            \rew(e'_{ij})   &\qquad\eqdef\qquad  \rew(i,n)+\rew(n,j)\\
            \dur(e'_{ij})   &\qquad\eqdef\qquad  \dur(i,n)+\dur(n,j)
        \end{align*}

	We first prove that $M$ and $\auxM$ have the same mean payoff value from every state $s\neq n$. Note that if $n$ was not part of a BSCC, 
	then the probability of reaching a BSCC is still preserved by our construction. This is because a path from $s$ to a BSCC in $M$ can be mapped to a path in $\auxM$ by replacing a sequence of edge $(i,n)(n,j)$ by $e'_{ij}$. This establishes a one-to-one correspondence between paths in $M$ and $\auxM$, which preserves the probability. 
	If $n$ is in a BSCC in $M$, then $n$ cannot be the only state in a BSCC due to the assumption that $\probm(n,n)=0$. 

        Let $s'$ be another state in the same BSCC as $n$. We prove that the $s'$-cycle mean-payoff value is preserved in the BSCC containing $n'$ in $\auxM$. The $s'$-cycles that do not involve the state $n$ are unchanged and therefore have the same probability, total reward and total duration.
	The $s'$-cycles containing the state $n$ can be mapped to a $s'$-cycle in $\auxM$ by replacing edges $(i,n)(n,j)$ by $e'_{ij}$. The mapping preserves the probability, reward and duration. Therefore, the expected $s'$-cycle mean-payoff values are the same in $M$ and $\auxM$.
	
	Note that $\auxM$ has multiple edges between pairs of state and by applying Lemma \ref{lem:edge-collapse} for every such pairs of state $i,j$, these can be replaced by one single edge to obtain a new Markov chain which is exactly $M'$ with the same value. Therefore, $M$ and $M'$ have the same value from all states $s\neq n$.
\end{proof}

\subsection{Loop Elimination}
	The loop-elimination step takes as input a Markov chain with states $\{1,\dots,n\}$ and produces a Markov chain $M'$ with states $\states'=\states$ such that for every state $i$, either $\probm'(i,i)=0$ or $\probm'(i,i)=1$ . %
        In other words, the algorithm eliminates self-loops on all transient states while preserving the mean-payoff value from the initial state $1$. 
        For every state $i,j$ such that $\probm(i,i)\neq 1$ and $i\neq j$, the values of probabilities, rewards, and durations of outgoing transition from $i$ to $j$ are updated as follows to obtain $M'$ (see also \cref{fig:loop_elim_full}).
	\begin{align*}
	\probm'(i,j) &\qquad\eqdef\qquad \frac{\probm(i,j)}{\sum_{k\neq i} \probm(i,k)} \\
	\rew'(i,j)   &\qquad\eqdef\qquad \frac{ \probm(i,i) }{ \sum_{k\neq i} \probm(i,k)}\rew(i,i) + \frac{\probm(i,j)}{\sum_{k\neq i} \probm(i,k)} \rew(i,j) 		\\
	\dur'(i,j)   &\qquad\eqdef\qquad \frac{ \probm(i,i) }{ \sum_{k\neq i} \probm(i,k)}\dur(i,i) + \frac{\probm(i,j)}{\sum_{k\neq i} \probm(i,k)} \dur(i,j) 	
	\end{align*}

\loopelim*
	
\begin{proof}
        Consider the Markov chain $M$ and let $n$ be the state whose loop is eliminated.
        We define an intermediate Markov chain $M''$ that replaces the self-loop by countably infinite length-$2$ paths via a new auxiliary state, each of which represents a fixed number of iterations of the loop.
        That is $M''$ is obtained from $M$ by adding a new state $n'$ and
        \begin{itemize}
            \item Every original edge between states $i,j\neq n$ have the same probability, reward and duration as in $M$.

            \item For every $\ell\ge 0$ there is a new edge $e_\ell$ between states $n$ and $n'$.
        with probability
        $\probm(e_\ell)=\probm(n,n)^{\ell}(1-\probm(n,n))$, reward
	$\rew(e_\ell)=\ell\cdot\rew(n,n)$ and duration $\dur(e_\ell)=
	\ell\cdot\dur(n,n)$.
	
        \item For every original edge $(n,j)$ with $j\neq n$, there is an edge $(n',j)$ with
        probability $\frac{\probm(n,j)}{1-\probm(n,n)}$
        and the same reward and duration as $(n,j)$.
        \end{itemize}
        See also \cref{fig:loop_elim_full} in the middle.
	Note that if $n$ was not part of a BSCC, 
	then the probability of reaching a BSCC is still preserved by our construction. This is because a path from $s$ to a BSCC in $M$ can be mapped to a path in $\auxM$ by replacing a $k$-fold iteration of the loop followed by a step $n\to i$, by the path that first takes edge $e_{k}$ and then $n'\to i$.
        This establishes a one-to-one correspondence between paths in $M$ and$\auxM$ that preserves the probability of reaching any fixed state.
	 
	If $n$ is in a BSCC in $M$, then $n$ cannot be the only state in a BSCC due to the assumption that $\probm(n,n)\neq 1$. 
        Let $s'$ be another state in the same BSCC as $n$. We prove that the $s'$-cycle mean-payoff value are equal in both $M$ and $\auxM$. 
        The $s'$-cycles that do not involve the state $n$ are unchanged and therefore have the same probability, total reward and total duration.
	The $s'$-cycles containing the state $n$ can be mapped to a $s'$-cycle in $\auxM$ by replacing edges $(n,n)^k$ by $e_{k}$ and $(n,j)$ by $(n',j)$.
        The probability of the $s'$-cycle in $M$ would be $p\cdot\probm(n,n)^k\probm(n,j)$, where $p$ is the product of the rest of the edges in the cycle.
        In $\auxM$, the probability of the same cycle would be $p\cdot\probm(n,n)^{k}(1-\probm(n,n)) \frac{\probm(n,j)}{1-\probm(n,n)}$, which is the same. 
        \ptnote{improve this?}
        It is also easy to see that the total reward and duration of the cycles are the same in $M$ and $\auxM$. 
        Therefore, the expected $s'$-cycle mean-payoff values are the same in $M$ and $\auxM$.
	
	If $M$ has a bound on reward on unit duration $B$ then the same bound applies to $\auxM$. The second assumption is also true as the expected reward and duration between $n$ and $n'$ is finite as it can be written as a geometric series, which is used to write the update in the loop elimination update. Therefore, we can apply Lemma \ref{lem:edge-collapse}, all edges $e_{\ell}$ can be combined to get a single edge while preserving the mean-payoff value. 
        \ptnote{WIP, fix lemma first}
	We can then apply the state elimination algorithm to eliminate state $n'$ and by \cref{lem:state-elim}, the mean-payoff value is still preserved from all states. This proves that we can eliminate the loop on one state, and in doing so we do not introduce a loop on any other state unless it was already present. 
	By iteratively doing this to all transient states with a loop, we can eliminate loops on all states to obtain exactly $M'$ described in the loop elimination updates. Therefore, $M$ and $M'$ have the same mean-payoff value from all states.  
\end{proof}
\begin{figure*}[t]
  \centering
  \input{fig/le-full.tikz}
  \caption{Loop elimination: On the left is (part of the) Markov chain $M$ before eliminating the self-loop in vertex $n$; On the right is the resulting chain $M'$. In the middle is the intermediate chain $M''$ with the countably infinite edges between $n$ and auxiliary state $n'$. Taking the $\ell$th edge represents taking the loop $\ell$ times.}
  \label{fig:loop_elim_full}
\end{figure*}


\subsection{Computing Mean-payoff Values} 
Note that a Markov chain obtained as the output of the loop-elimination algorithm satisfies the
conditions on the input of the state-elimination algorithm. Therefore, we can apply loop elimination followed by state elimination to every transient state other than the initial state $1$ while preserving the mean-payoff value from the initial state. After at most $n-1$ iterations, we will be left with a Markov chain where all states of a BSCC are merged together to a single state and the initial state is the only transient state (if it is not part of a BSCC). The mean payoff value in these case can be computed as follows: 

\begin{itemize}
	\item Case 1. The initial state is in a BSCC, which will be merged to a single state with a self loop. Therefore the mean-payoff value will be $\rew(1,1)/\dur(1,1)$.
	\item Case 2. The initial state $1$ is a transient state and all other states are absorbing state which corresponds to a merged BSCC. 
	For every state $i,\neq 1$, the mean payoff value of state $i$ is $v_i= \rew(i,i)/\dur(i,i)$, similar to the case above. The value of state $1$ will be $\sum_i\probm(1,i)v_i$.  
\end{itemize}

Note that the loop-elimination and state-elimination procedures run in polynomial time and the number of iterations of these sub-routines are bounded by the number of states of the Markov chain. Therefore, the algorithm takes time polynomial in the size of the Markov chain.







	
















==> sec.solan.tex <==




\begin{restatable}{lemma}{solan}
\label{lem:solan}
Consider any pair of strategy profiles $\sigma\in \BSB{\vec{b}}$ and $\sigma'\in \BSB{\vec{b}}$, such that $\rdist(\sigma,\sigma')<(4N)^{-1}$.
Then, $v_{\sigma'}\in [v_{\sigma}-\gamma,v_{\sigma}+\gamma]$, where $\gamma=9\cdot N\cdot \rdist(\sigma,\sigma')C$.
\end{restatable}


\ptnote{below is proof of repr lemma}
On the other hand, if we have some $\epsilon$-Nash equilibrium $\sigma$ wrt $\BSB{\vec{b}}$, for some $\epsilon\geq 0$ then player $i$, for all $i$, can not get more than $\epsilon$ better by following any strategy $\sigma_i$ in $\BSP{i}{\vec{b}}$ than whatever they get without changing by definition. Let $\sigma'$ be any strategy profile arising from perturbing $\sigma$ slightly and we will argue that it is a $\epsilon'$-Nash equilibria for 
\[\epsilon'=18\cdot N\cdot \rdist(\sigma,\sigma')C+\epsilon.\]
For any strategy $\sigma_i$ for player $i$, we have that the outcome for player $i$ when players play $\sigma'[\sigma_i]$ only differs slightly from when they play $\sigma[\sigma_i]$ by the lemma, which, by definition only differs slightly from when they play $\sigma$, which in turn only differs slightly from when they play $\sigma'$ by the lemma. Hence, inserting the numbers, the outcome for player $i$ when players play $\sigma'[\sigma_i]$ differs by at most $\epsilon'=18\cdot N\cdot \rdist(\sigma,\sigma')C+\epsilon$ from when they play $\sigma'$. 


==> thm.big-number-solutions.tex <==



\begin{proof}
We apply 
\cite[Thm~14.16]{BPR2006}
to 
\[\phi(x_1^1,\dots,x_{n_1}^1)\eqdef 
\forall x_1^2,\dots,x_{n_2}^2\exists\dots x_1^k\dots,x_{n_k}^k: \varphi(x_1^1,\dots,x_{n_1}^1,x_1^2\dots,x_{n_k}^k)\]
which gives us a quantifier-free expression of  $\phi$. This expression of $\phi$ uses polynomials of degree at most $d'\eqdef d^{\prod_{i=2}^k O(n_i)}$ with integer coefficients, each of bit-size at most $\tau'\eqdef \tau d^{\prod_{i=1}^k O(n_i)}$.
We then apply 
\cite[Thm~13.10]{BPR2006}
to $\phi$, giving us a ``univariate representation'' of each of the numbers we will use for $x_i'$ 
(the theorem itself only states that we get approximations, but the complexity analysis of the algorithm states that it is equally fast to get exact solutions, using some additional steps). 
For each $i$, this univariate representation for $x_i$ consists of a fraction of two polynomials $p_i(x)/q(x)$ and an additional polynomial $f$ ($q$ and $f$ are coprime). The number $x_i$ is then $p_i(t)/q(t)$ where $t$ is a root of $f$. These polynomials each is of degree at most $d''\eqdef (2d'+6)^{n_1}\leq (2d)^{\prod_{i=1}^k O(n_i)}$ (we get to ignore the $6$ because of the $O$'s. We can't ignore the 2 in case $d$ was 1) with integer coefficients of bit-size at most $\tau''\eqdef \tau d^{\prod_{i=1}^k O(n_i)}$. 
For each $i$, we apply
\cite[Lem.~15]{BPR2006}
to $f$, $p_i$ and $q$, giving us a square-free univariate polynomial $p'_i$ such that $p'_i(x_i)=0$. This polynomial has degree at most $d'''\eqdef 2d''=(2d)^{\prod_{i=1}^k O(n_i)}$ and the bitsize representation of the integer coefficients is at most $\tau'''\eqdef 2d''\tau''+7d''\log d''=\tau (2d)^{\prod_{i=1}^k O(n_i)}$.

For any univariate polynomial $p(x)=a_n x^{n-1}+a_{n-1} x^{n-2}+\dots+a_1 x+a_0$, then $r\neq 0$ is a root iff $1/r\neq 0$ is a root of $a_n 1/(x^{n-1})+a_{n-1} (1/x^{n-2})+\dots+a_1 1/x+a_0$ or equally $p'(x)\eqdef a_n +a_{n-1} x+\dots+a_1 x^{n-2}+a_0 x^{n-1}$. Therefore, if $U$ is an upper bound on the absolute largest root in $p$, then $1/U$ is a lower bound for how small the absolute smallest non-zero root can be in $p'$. 
We can bound $U\le 1+\max\left(\abs{\frac{a_{n-1}}{a_{n}}},\abs{\frac{a_{n-2}}{a_{n}}},\dots \abs{\frac{a_{0}}{a_{n}}}\right)$
\cite{Cau1828}
and so
get that $2^{-\tau'''}\leq |x_i'|\leq 2^{\tau'''}$, because the largest integer represented with $x$ bits is $2^{x}-1$.
 \end{proof}

